EduCOR: An Educational and Career-Oriented Recommendation Ontology

With the increased dependence on online learning platforms and educational resource repositories, a unified representation of digital learning resources becomes essential to support a dynamic and multi-source learning experience. We introduce the EduCOR ontology, an educational, career-oriented ontology that provides a foundation for representing online learning resources for personalised learning systems. The ontology is designed to enable learning material repositories to offer learning path recommendations, which correspond to the user's learning goals, academic and psychological parameters, and the labour-market skills. We present the multiple patterns that compose the EduCOR ontology, highlighting its cross-domain applicability and integrability with other ontologies. A demonstration of the proposed ontology on the real-life learning platform eDoer is discussed as a use-case. We evaluate the EduCOR ontology using both gold standard and task-based approaches. The comparison of EduCOR to three gold schemata, and its application in two use-cases, shows its coverage and adaptability to multiple OER repositories, which allows generating user-centric and labour-market oriented recommendations.

==> sections/coreLP.tex <==
\subsection{Learning Path pattern}

\begin{tabular}{ |p{3cm}|p{12cm}|  }
 \hline
 Name & Learning Path pattern\\
\hline
 Intent & This pattern demonstrates the learning path \\
 \hline
Description  &  The learning path pattern is proposed to arrange individual recommendations into full learning sequences. Those sequences target namely a complex skill, which is not likely to be met by learning only one Knowledge Topic. Path generation includes the definition off all knowledge topics that are required to reach a certain skill, based on the learning objectives and goals, as well as the recommendation requirements. \\
 \hline
Concepts Presented & Learning Path, Knowledge Topic, Educational Resource, Learning Goal, Learning Objective, Recommendation \\
\hline
Axiomatization &   \begin{itemize}
\item Multiple learning paths with the same learning goal have different weights based on the Recommendation Requirements. 
\item A learning path can not start with an advanced topic and end with a basic one if both topics are in the same domain. 

Learning Path LP, ki knowledge topic in i-th order in the learning path order, li the level difficulty of ki
If LP=(k1, ..., ki, ..., kn) then l1 $\leq$ ln


\end{itemize}\\ 

\hline
Example Use-Case & A hybrid recommender system is designed to integrate three recommendation resources: the teacher, domain and similar users, to generate a study recommendation. The recommender suggests next steps in the learning process, based on the current learning state and the knowledge extracted from the teacher and the domain. However, the generation of next-step learning-recommendation is not possible for more than one step ahead. This is due to the lack of a clear definition of ordering future learning steps, as well as determining the content of those steps. Through the use of the proposed Learning Path Pattern, such definitions can be found, to support the recommender system in defining not only the next learning step, but rather a set of multiple steps ahead. Recommending an ordered path of learning topics offers new value-added to the learner and the system. For the learner, defining a full learning path makes it easier to see the rationale behind studying the first topics in the path. This becomes very important when the first steps are basic concepts, which learners tend to overlook when searching for an advanced-level information. For the system itself, the definition of a learning path enables creating a virtual learning strategy and connecting it with a certain learning goal. By comparing the path that has been recommended to the learner with the actual path that the learner chooses, and then the evaluation results of the learning process (e.g. through test scores), the system can automatically evaluate the validity of a certain recommended learning path and its role in achieving a mastery level of the targeted learning goal. This can enable the system of learning how to adjust the learning path according to certain criteria, e.g. the user preferences or previous experiences. \\
 \hline
\end{tabular}

  \begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{images/learningpathpattern.png}
    \caption{Learning Path pattern}
    \label{fig:my_label}
\end{figure}

\newpage

\begin{tabular}{ |p{3.5cm}|p{2.8cm}|p{10cm}|  }
 \hline
Property & Expected Type & Description \\
\hline
Learning Path & List & An ordered list of recommendations, which is personalized to the needs of a certain user and target the accomplishment of a complex skill. It has as a final point a learning goal. \\
\hline
Recommendation & Knowledge Topic, Exercise, Other& The output of the recommendation system. The algorithm that reads the recommendations and uses information of the user, ratings and any available rules, in order to generate a sequence of multiple recommendations \\
\hline
LearningGoal & Knowledge Topic &The reach point of a learning path. The completion of a set of knowledge topics which can lead to mastering a skill. \\
\hline
LearningObjective & Text &The learning outcomes and demonstrable skills or knowledge that will be acquired by a student as a result of the learning goal.\\
 \hline
KnowledgeTopic & Knowledge Topic & A single node representing a learning module based on the domain ontology. It contains all the learning material for the specific learning module. For example, a knowledge topic can be the “Quadratic equations” which could contain all the learning material (theory, exercises etc) for this topic. \\
\hline
EducationalResource & URL & A coursebook, or an online course, MOOC etc which defines the source of the OER. It is tightly linked to the domain ontology. \\
\hline
definesLearningPath & List & Represents the algorithm, which is intended to generate a full learning path from individual recommendations. The algorithm takes into account the recommendation requirements from the Recommender Pattern when ordering the topics in the learning path.\\
\hline
hasLearningGoal & Knowledge Topic, Test & The learning path generation targets a specific learning goal. Therefore, this relation represents the role that learning gals and objectives in the generation of the learning path. \\
\hline
hasLearningObjective & Text & \\
\hline
consistsOfKnowledge & Knowledge Topic & Represents the actual content of the learning path, which is the recommended Knowledge Topics to the learner.\\
\hline
hasEducationalResource & URL & Determines the sources, online or offline, for each recommended knowledge topic.\\
\hline

\end{tabular}

==> sections/coreTEST.tex <==
\subsection{Test pattern}


\begin{tabular}{ |p{3cm}|p{9cm}|  }
 \hline
 Name & Test pattern\\
\hline
 Intent & This pattern demonstrates the test \\
 \hline
Description  &  \\
 \hline
Concepts Presented & Learning Path, Knowledge Topic, Educational Resource, Learning Goal, Learning Objective, Recommendation \\
\hline
Example & \\
 \hline
\end{tabular}

\begin{figure} [h!]
    \centering
    \includegraphics[width=0.7\textwidth]{images/testpattern.png}
    \label{fig:my_label}
\end{figure}




\begin{tabular}{ |p{3.5cm}|p{3cm}|p{9cm}|  }
 \hline
Property & Expected Type & Description \\
\hline
Test & & A test consists of one or many exercises, which have questions and answers. It is the way to evaluate student knowledge for a (set of) knowledge topic(s). It is linked to one or many skills and can have some educational requirements. \\
\hline
Timestamp &  & The unique timestamp for the test result. It is generated automatically once a user completes a test. \\
\hline
LearningGoal & Knowledge Topic & The reach point of a learning path. The completion of a set of knowledge topics which can lead to mastering a skill. \\
\hline
LearningObjective & Text &The learning outcomes and demonstrable skills or knowledge that will be acquired by a student as a result of the learning goal.\\
 \hline
KnowledgeTopic & & A single node representing a learning module based on the domain ontology. It contains all the learning material for the specific learning module. For example, a knowledge topic can be the “Quadratic equations” which could contain all the learning material (theory, exercises etc) for this topic. \\
\hline
EducationalResource & & A coursebook, or an online course, MOOC etc which defines the source of the OER. It is tightly linked to the domain ontology. \\
\hline
defines & & \\
\hline
has & & \\
\hline
consistsOf & & \\
\hline
hasEducationalResource & & \\
\hline

\end{tabular}

==> sections/coreUserP.tex <==
\subsection{User Profile Pattern}

\begin{tabular}{ |p{3cm}|p{9cm}|  }
 \hline
 Name & User Profile Pattern\\
\hline
 Intent & A pattern that represents the user in the system. \\
 \hline
Description  &  User pattern includes all the information that the system requires about the user in order to make a decision (e.g. a recommendation). The user pattern is designed to account for academic and psychological factors that influence the learning process of the user. It also includes the user defined values (e.g. preferences) that is taken into consideration in the recommendation generation\\
 \hline
Concepts Presented & User, Learning Preference, Learning Goal, Psychological Construct, Psychological Indicator, Dynamic Indicator, Static Indicator, Academic Parameter, Academic Indicator. \\
\hline
Example & \\
 \hline
\end{tabular}


\begin{figure} [h!]
    \centering
    \includegraphics[width=0.7\textwidth]{images/UserProfilePattern.png}
    \caption{User Profile pattern}
    \label{fig:my_label}
\end{figure}




\begin{tabular}{ |p{3.5cm}|p{3cm}|p{9cm}|  }
 \hline
Property & Expected Type & Description \\
\hline
User & Person & The data that defines the user, whether anonymously or clearly, such as UserID, contact information, etc.  \\
\hline
Learning Preference & Text & Represents the user-defined values that should influence the recommendation. Such values include the type of learning material, its length, ratio of exercises, among others. Learning preferences have also the potential to be learned by the system from the accumulative user behaviour.\\
\hline
Psychological Construct & & A high level representation of psychological, measurable, state of mind, e.g. tiredness, focus, etc.\\
\hline
Psychological Indicator & & The actual representation of a certain measure, which is meant to represents a psychological aspect, such as the time needed to answer a question, number of clicks, etc.\\
\hline
Dynamic Indicator & & An indicator that is expected to change with time, such as the time needed to answer a question. \\
\hline
Static Indicator & & An indicator that is not expected to change frequently, such as the preference of a learning-material-type. \\
\hline
Academic Parameters & & High level representation of academic measurable performance, e.g. course mastery level. \\
\hline
Defines & & Represents the psychological scoring algorithm, which translates the indicators into high-level constructs. It defines the indication and thus the use of each indication in the decision making algorithm, e.g. the recommender.\\
\hline
measures & & The measurement method used to quantify the indicator and capture its value, whether from the user behaviour or interaction with the system, such as measuring the time for answering a question. \\

\end{tabular}

==> sections/methodology.tex <==
\section{Methodology}


